Structural transitions of calcium carbonate by molecular dynamics simulation

Calcium carbonate plays a crucial role in the global carbon cycle, and its phase diagram has always been of significant scientific interest. In this study, we used molecular dynamics (MD) to investigate several structural phase transitions of calcium carbonate. Using the Raiteri potential model, we explored the structural transitions occurring at a constant pressure of 1 bar with temperatures ranging from 300 K to 2500 K, and at a constant temperature of 1600 K with pressures ranging from 0 to 13 GPa. At increasing temperatures, the transitions calcite, CaCO$_3$-IV, and CaCO$_3$-V are observed and characterized. Within the calcite structure, CO$_3^{2-}$ ions are ordered between layers. As temperature increases, the calcite to CaCO$_3$-IV transition occurs, determining the partial disordering of CO$_3^{2-}$ ions. At a higher temperature, CaCO$_3$-IV transforms into CaCO$_3$-V. By applying free energy analysis, we have classified the last transition as a continuous order-disorder phase transition. At a temperature of 2000 K, it appears a `disordered CaCO$_3$' structure, characterized by low order within the calcium and carbonate sublattices and the free rotation of CO$_3^{2-}$ ions. At increasing pressures, two calcium carbonate transformations were observed. At $P=$ 2 GPa, the CaCO$_3$-IV phase undergoes a phase transition into CaCO$_3$-V, demonstrating that the model can describe the transition between these two phases as pressure and temperature-driven. Another phase transition was detected at $P=$ 4.25 GPa -- CaCO$_3$-V transits into the recently discovered CaCO$_3$-Vb phase. This transition is classified as a first-order phase transition by structural analysis and free energy-based arguments.

==> latexmkrc <==
# This shows how to use the xr package with latexmk.
# John Collins 2023-03-29
#
# The xr package ("a system for eXternal References") is used by a document
# to make references to sections, equations, etc in other external
# documents. 
# The definitions in this file enable latexmk to apply latexmk to
# automatically update an external document whenever its .tex file changes,
# so that the references in the main document stay up to date.

# Notes:
#    1. This version is defined to put the files from the compilations of
#       the external documents into a defined subdirectory, to segregate
#       potentially many generated files from the main document
#       directories. 
#    2. But for latexmk's custom dependency mechanism to be used, as here,
#       the aux file from compilation of a subdocument must be generated in
#       the same directory as the corresponding source .tex file.  So the
#       .aux file is copied.
#    3. It is assumed that the external documents are to be compiled by
#       pdflatex.  This can be changed, of course, by changing the '-pdf'
#       option given to the invoked latexmk to whatever is needed.
#    4. An ideal implementation would also ensure that recompilation of an
#       external document also happens whenever any of its other source
#       files changes.  But this is not done in the present version, and
#       would probably entail either the use of internal latexmk variables
#       or extra enhancements to latexmk.
#    5. The code uses subroutines copy and fileparse that are loaded by
#       latexmk from the Perl packages File::Copy and File::Basename.
#    6. It also uses some not-yet-documented features of latexmk: an array
#       variable @file_not_found and subroutines popd, pushd, and
#       rdb_add_generated. 


#--------------------
# Configurable choices for compilation of external documents

# Subdirectory for output files from compilation of external documents:
$sub_doc_output = 'output-subdoc';

# Options to supply to latexmk for compilation of external documents:
@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

#--------------------

# Add a pattern for xr's log-file message about missing files to latexmk's
# list.  Latexmk's variable @file_not_found is not yet documented.
# This line isn't necessary for v. 4.80 or later of latexmk.
push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {
               # In this case, .aux file generated by pdflatex isn't in same
               # directory as the .tex file.
               # Therefore:
               # 1. Actual generated aux file must be listed as produced by this
               #    rule, so that latexmk deals with dependencies correctly.
               #    (Problem to overcome: If $sub_dir_output is same as $aux_dir
               #    for the main document, xr may read the .aux file in the
               #    aux_dir rather than the one the cus dep is assumed by latexmk
               #    to produce, which is in the same directory as the .tex source
               #    file for this custom dependency.)
               #    Use not-yet-documented latexmk subroutine rdb_add_generated
               #    to do this:
               # 2. A copy of the .aux file must be in same directory as .tex file
               #    to satisfy latexmk's definition of a custom dependency.
             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}

==> multiple.tex <==
main.tex toplevelfile
SI.tex toplevelfile

